What Went Wrong? Explaining Overall Dialogue Quality through Utterance-Level Impacts

Improving user experience of a dialogue system often requires intensive developer effort to read conversation logs, run statistical analyses, and intuit the relative importance of system shortcomings. This paper presents a novel approach to automated analysis of conversation logs that learns the relationship between user-system interactions and overall dialogue quality. Unlike prior work on utterance-level quality prediction, our approach learns the impact of each interaction from the overall user rating without utterance-level annotation, allowing resultant model conclusions to be derived on the basis of empirical evidence and at low cost. Our model identifies interactions that have a strong correlation with the overall dialogue quality in a chatbot setting. Experiments show that the automated analysis from our model agrees with expert judgments, making this work the first to show that such weakly-supervised learning of utterance-level quality prediction is highly achievable.

==> 02-Task.tex <==
\section{Task Formulation }
\label{sec:task}

Our goal is to automatically infer the impact of utterance-level interactions on conversation quality. Formally, given a dataset of pairs $\{x_i, y_i\}$ where $x_i$ is the $i$th conversation and $y_i$ is a real number denoting its quality, the task is to assign a continuous-valued score $s_{ij}$ to each utterance $u_{ij}$ in the dataset. In theory, each utterance score $s_{ij}$ should represent the quantitative impact of the $j$th utterance on the quality $y_i$ of the $i$th conversation, such that the following holds:

\begin{equation}
\label{task}
    \forall i \hspace{1mm} \forall j\leq N_i \sum\limits_{k=1}^j s_{ik} = y_{ij} 
\end{equation}

% \begin{equation}
% \label{task}
%      
% \end{equation}

\noindent where $y_{ij}$ is the overall quality of utterance 1 to utterance $j$ of conversation $x_i$ and conversation $x_i$ has $N_i$ total utterances. 

Although the task objective presented in equation \ref{task} is mathematically straightforward, an automatic solution to this task is nontrivial, since labels $y_{ij}$ are not given. As a result, 
the model must infer utterance-level scores based only on quality labels $y_i$ of entire conversations.

% \begin{equation}
%     \forall i \sum\limits_{k=1}^{N_i} s_{ik} = y_i 
% \end{equation}

In fact, even direct verification of equation \ref{task} for model evaluation is infeasible, since it not only requires the subjective assessment of quality, but also high internal consistency between quality judgements of each conversation segment.
In section \ref{sec:evaluation}, we describe how we approximated our task as a ranking problem in order to evaluate our model against expert judgements. 

% \begin{equation}
%     \forall i \sum\limits_{k=1}^{N_i} s_{ik} = y_i 
% \end{equation}
% \noindent where conversation $x_i$ has $N_i$ total utterances. 

% Although this relationship is most intuitively applied to complete conversations, there is no requirement in reality that conversations have to be completed before a quality judgement is possible. Indeed, any subsection of a conversation can be judged for quality and, with this perspective, the general formulation of the task objective is as follows:


% \subsection{Comparison to Previous Work}

% Previous works have explored similar tasks of classifying utterances on a binary scale \cite{choi19}. However, it is important to be able to assess relative importance between utterances on a fine-grained level for many practical applications, thus leading to the formulation of this task as an utterance-level regression.

% * More to add

